On Reporting Durable Patterns in Temporal Proximity Graphs

Finding patterns in graphs is a fundamental problem in databases and data mining. In many applications, graphs are temporal and evolve over time, so we are interested in finding durable patterns, such as triangles and paths, which persist over a long time. While there has been work on finding durable simple patterns, existing algorithms do not have provable guarantees and run in strictly super-linear time. The paper leverages the observation that many graphs arising in practice are naturally proximity graphs or can be approximated as such, where nodes are embedded as points in some high-dimensional space, and two nodes are connected by an edge if they are close to each other. We work with an implicit representation of the proximity graph, where nodes are additionally annotated by time intervals, and design near-linear-time algorithms for finding (approximately) durable patterns above a given durability threshold. We also consider an interactive setting where a client experiments with different durability thresholds in a sequence of queries; we show how to compute incremental changes to result patterns efficiently in time near-linear to the size of the changes.

==> aggregate.tex <==
\section{Aggregate-Durable Pairs}
\label{sec:aggregate}

In this section, we consider reporting aggregate-durable pairs under SUM function in Section~\ref{subsec:sum} and UNION function in Section~\ref{subsec:union}.

\subsection{SUM}
\label{subsec:sum}

We start by describing a data structure that allows us to find efficiently the total length of all intersections of a query interval with a given set of intervals. Then we use this data structure to decide if a pair is $\tau$-durable pair. Our data structure might also return ``yes'' if $p,q$ is a $\tau$-durable $\eps$-pair, but return ``no'' in all other cases.
Then we show how to use this data structure to report all $\tau$-durable pairs.

\smallskip \noindent {\bf Primitive: Interval-SUM-durability.} Given a set of intervals $\mathcal{I}$, the goal is to construct a data structure for $\mathcal{I}$ such that for any query interval $I'$ and $\tau >0$, whether $\sum_{I \in \mathcal{I}}|I\cap I'|\geq \tau$ can be decided efficiently.
%
%\begin{definition}[Detect-SUM-durability]
%    Given a set of intervals $\mathcal{I}$, the goal is to construct a data structure for $\mathcal{I}$ such that given a query interval $I'$ and a durability parameter $\tau$, we check whether $\sum_{I \in \mathcal{I}}|I\cap I'|\geq \tau$.
%\end{definition}
%\begin{itemize}
%    \item {\bf Compute-SUM-durability.} Given a set of intervals $\mathcal{I}$, the goal is to construct a data structure for $\mathcal{I}$ such that given a query interval $I'$ and a durability parameter $\tau$, we check whether $\sum_{I \in \mathcal{I}}|I\cap I'|\geq \tau$.
%\end{itemize}
%The data structure below is referred as {\sc ComputeSum}.
We construct a variation of interval tree $\IT$ over the set of intervals $\I$, and store for each node $u \in \IT$: 
\begin{itemize}[leftmargin=*]
    \item $|u|$, i.e., the total number of intervals stored at $u$;
    \item $\sum_{I \in u} |I|$, i.e., the total length of intervals stored at $u$;
    \item $\sum_{I \in u} I^+$, i.e., the sum of right endpoints of intervals stored at $u$;
    \item $\sum_{I \in u} I^-$, i.e., the sum of left endpoints of intervals stored at $u$.
\end{itemize}
The interval tree $\IT$ can be constructed in $O(n\log n)$ time and uses $O(n\log n)$ space. After issuing a query interval $I'$ to $\IT$, we obtain $O(\log n)$ canonical set of nodes, where each node $u$ must fall into one of the following types: (1) every $I \in u$ completely covers $I'$; (2) $I'$ completely covers every $I \in u$; (3) every $I \in u$ partially intersects $I'$ with $I^+ \in I'$; (4) every $I \in u$ partially intersects $I'$ with $I^- \in I'$. Then, we can rewrite the SUM-durability of $I$ as the sum of aggregation over every canonical node $u$: %\begin{align*}
%    \sum_{I \in \I} |I \cap I'| & = \sum_{u} \sum_{I %\in u} |I \cap I'|
%\end{align*}
%where
\begin{displaymath}
\sum_{I \in \I} |I \cap I'| = \sum_{u} \sum_{I \in u} |I \cap I'| =\sum_u \left\{ \begin{array}{ll}
|u| \cdot |I'| & \textrm{if (1)}\\
\sum_{I \in u} |I| & \textrm{if (2)}\\
 \sum_{I \in u} I^+ - |u| \cdot I'^- & \textrm{if  (3)} \\
|u| \cdot I'^+ - \sum_{I \in u} I^- & \textrm{if (4)} \\
\end{array} \right.
\end{displaymath}
In this way, we can compute $\sum_{I\in S_I}|I\cap I_p|$ in $O(\log n)$ time. 

\paragraph{Data structure.}
We first construct $\DTC$ as described in Section~\ref{sec:tau-durable-ball} with slight modifications.
Recall that $\DTC$ is a two-level data structure that consists of a cover tree and an interval tree for every node of the cover tree. For each canonical node of every interval tree of $\DTC$, we store points in decreasing order with respect to their right interval endpoint, i.e., $p<q$ if $I_p^+<I_q^+$.
For each node in the cover tree of $\DTC$, we construct $\IT$ as described above.
If $\bigcirc_j$ is the ball of a node $v_j$ in the cover tree of $\DTC$, we construct $\IT$ over the points of $P$ in $\bigcirc_j$.
By slightly abusing the notation we use $\bigcirc_j$ to denote both the ball of a node $v_j$ and the points of $P$ stored in $v_j$. We also define $\IT(\bigcirc_j, I)$ as the sum of the lengths of the intersection of $I$ with intervals whose points lie in $\bigcirc_j$, i.e. $\IT(\bigcirc_j, I)=\sum_{q\in \bigcirc_j} |I_q\cap I|$.
Overall we can construct $\DTC$ along with the extended intervals trees $\IT$ in $O(n\log^2 n)$ time having $O(n\log^2 n)$ space. The query time is $O(\eps^{-O(\ddim)}\log^2 n)$.

\paragraph{High-level Idea.}
With the modified data structure $\DTC$, we can decide if a pair is $\tau$-durable efficiently. Unfortunately, if we use this data structure for every pair $(p,q) \in P \times P$, we would end up with an $O(n^2)$ time algorithm. Instead, for each point $p\in P$ we use the space decomposition from the previous sections to group the points, close to point $p$, whose time-intervals include $I_p^-$, into small balls. Then by visiting each point $q$ in a ball in decreasing order of their right time-interval endpoint, we make sure that when we find $q$ such that the pair $p,q$ is not $\tau$-durable then we can safely skip the current ball because there is no other $\tau$-durable pair to report.

\smallskip
\noindent {\bf Algorithm.} As preprocessing, we build the data structure $\DTC$ as described above. In Algorithm~\ref{alg:sum}, we visit each input point $p \in P$ and report $\tau$-SUM-durable pairs that contain $p$.
Recall that $\C_{p,j}$ is a canonical node of the cover tree in $\DTC$. We denote $\bigcirc_{p,j}$ as the corresponding ball of the node of the cover tree in $\DTC$.
%
\begin{algorithm}[t]
\caption{{\sc ReportSUMPair}$(p, \tau, \epsilon, \DTC)$}
\label{alg:sum}

$\C_{p} \gets \DTCQ(p,\tau,\eps/2)$\;
Assume $\C_{p} = \{\C_{p,1}, \C_{p,2}, \cdots, \C_{p,k}\}$\;
\ForEach{$j \in [k]$}{
    \ForEach{$q\in \C_{p,j}$ in descending order of $I_q^+$}{
        $s=0$\;
        \ForEach{$i \in [k]$}{
             \If{$\dist(\textsf{rep}_i, \textsf{rep}_j) \le 1+ \frac{\epsilon}{2}$}{
                $s=s+\IT(\bigcirc_{p,i}, I_p\cap I_q)$\;
             }
        }
        \lIf{$s\geq \tau + 2\cdot|I_p\cap I_q|$}{
            Report$(p,q)$}\lElse{break}
    }
}
\end{algorithm}
%
%
\begin{comment}
\begin{algorithm}
\caption{{\sc ReportPair}$(p, \tau, \epsilon, \DTC)$}
\label{alg:offline-2}

$\C_{p} \gets \DTCQ(p,\tau,\eps/8)$\;
Assume $\C_{p} = \{\C_{p,1}, \C_{p,2}, \cdots, \C_{p,k}\}$\;
\ForEach{$j \in [k]$}{
    $X \gets \emptyset$\;   
    \ForEach{$i \in [k]$}{
        \lIf{$\dist(\textsf{rep}_i, \textsf{rep}_j) \le 1+ \frac{\epsilon}{2}$}{$X \gets X \cup \C_{p,i}$}
    }
    $\IT \gets$ (extended) interval tree built for $\{I_{q'}: q' \in X\}$\;
    Assume $\C_{p,j}$ is sorted by the right endpoint of the associated lifespan intervals decreasingly\; 
    \ForEach{$q \in \C_{p,j}$}{
        \If{$\textsc{\upshape ComputeSUM}(\IT, I_p \cap I_q) \ge \tau$}{
            \lIf{$I^-_p > I^-_q$}{Report $(p,q)$}
        }
        \lElse{\Return}
    }
}
\end{algorithm}
\end{comment}
%
Next, we focus on one input point $p \in P$. Similarly, we first 
run a $\tau$-durable ball query $\DTCQ(p,\tau, \epsilon/2)$ and obtain a canonical set of nodes $\C_p = \{\C_{p,1}, \C_{p,2},\ldots, \C_{p,k}\}$ for $k = O(\epsilon^{-\ddim})$.
Each $\C_{p,j}$ represents a node in the cover tree of $\DTC$ with diameter $\eps/2$.
For each such node $\C_{p,j}$ we get $O(\log n)$ canonical subsets of the points $P_{(p,j,\tau)}=\{p'\in P\cap \C_{p,j}\mid I_{p'}^+\geq I_p^-+\tau, I_{p'}^-\leq I_p^-\}$, i.e., the points in $C_{p,j}$ whose intervals sufficiently intersect $I_p$, running a query in the interval tree stored at $\C_{p,j}$, as explained in Section~\ref{sec:tau-durable-ball}.
With a slight abuse of notation, we often use $\C_{p,j}$ to denote $P_{(p,j,\tau)}$.
Observe that for each point $q \in \C_p$ returned, it is guaranteed that $\dist(p,q) \le 1+ \eps$, but not necessarily $\dist(p,q) \le 1$, due to the approximation.
%To abuse of notation, we often use $\C_{p,j}$ to denote the set of points lying inside the corresponding node whose intervals intersect $I_p^-$ (recall that we can find these points using the interval trees in the second level of $\DTC$). Recall that $\textsf{rep}_j$ is the representative point of node $\C_{p,j}$.

%Before proceeding to the reporting phase, we point out an important observation on the durable pairs $(p,q)$ if there exists any. Let $U$ be the witness set of $(p,q)$. As each point $q' \in U$ has distance at most $1$ from both $p,q$, there must be $q, q' \in \C_p$. Suppose $q \in \C_{p,j}$ and $q' \in \C_{p,i}$. Then, $\dist(\textsf{rep}_j, \textsf{rep}_i) < 1 + \frac{\eps}{2}$. Our reporting procedure exactly follows this critical observation.


Let $q$ be a point in $\C_{p,j}$ following the descending ordering by the right endpoint of intervals, as described above. We check if $p,q$ is a $\tau$-SUM-durable pair.
For each $\C_{p,i}$, if $\dist(\textsf{rep}_j,\textsf{rep}_i)\leq 1+ \eps/2$, we run a query in $\IT$ to find $\IT(\bigcirc_{p,i}, I_p\cap I_q)=\sum_{q'\in \bigcirc_{p,i}}|I_p\cap I_q\cap I_{q'}|$. In the end, if the total sum of all intervals in the nodes $\C_{p,i}$ with $\dist(\textsf{rep}_j,\textsf{rep}_i)\leq 1+\eps/2$, is at least $\tau+2\cdot|I_p\cap I_q|$,\footnote{We check if the sum is $\geq \tau+2\cdot|I_p\cap I_q|$ and not $\geq \tau$ because: i) When $i=j$, $\dist(\textsf{rep}_j,\textsf{rep}_i)=0\leq 1+\eps/2$, so we will consider $I_q$ in the sum; ii) When $p\in \bigcirc_{p,i}$, $\dist(\textsf{rep}_j,\textsf{rep}_i)\leq\dist(\textsf{rep}_j, p)+\dist(p,\textsf{rep}_i)\leq 1+\eps/2$, so we will consider $I_p$ in the sum.} we report $(p,q)$. If not, we stop traversing intervals in $\C_{p,j}$, as $\C_{p,j}$ does not contain any other point that can form a $\tau$-SUM-durable pair with $p$.
%
%
%We visit each canonical node in $\C_p$. For $\C_{p,j}$ visited, we find the set of points from other canonical nodes in $\C_p$ that have distance within $1 + \frac{\eps}{2}$ from $\C_{p,j}$ (line 4-6), denoted as $X$. We then build an extended interval tree on the lifespan intervals of points in $X$. Now, we are ready to identify $q$ from $\C_{p,j}$, and check whether $(p,q)$ is a durable pair. To avoid too many wasted invocations of {\sc ComputeSum} for points in $\C_{p,j}$, which actually do not form a $\tau$-SUM-durable pair with $p$, we use another trick by visiting points in $\C_{p,j}$ in a decreasing order of the right endpoint of its lifespan interval.
%
%\noindent When constructing the interval tree $\IT$, we can stored intervals in each node in decreasing order with respect to their right endpoint, thus avoid sorting $\C_{p,j}$ on the fly. Suppose point $q \in \C_{p,j}$ is visited. We invoke the procedure $\textsc{ComputeSum}$ for computing the aggregated durability of $I_p \cap I_q$. If the returned answer is greater than $\tau$, we report $(p,q)$ as a $\tau$-SUM-durable pair and continue visiting the remaining points in $\C_{p,j}$. Otherwise, we just stop and proceed to the next canonical node in $\C_p$. 
%
%
%
%We can show that all $\tau$-SUM durable pairs along with a few $\tau$-SUM durable $\eps$-pairs will be reported, so $|K_\tau\leq| \OUT\leq |K_{\tau}^\eps|$.
%
The correctness and complexity analysis are given in Appendix~\ref{appendix:aggregate}.

\begin{theorem}
    \label{thm:offlineSUM}
    Given a metric space $(P,\phi)$ of $n$ points, $\tau > 0$ and $\eps > 0$, the $\eps$-approximate \problemthree\ problem with SUM can be solved in $O(n\cdot(\eps^{-O(\ddim)}\log n+\log^2 n) + \OUTS \cdot \eps^{-O(\ddim)}\log^2 n)$ time, where $\ddim$ is the doubling dimension of $P$ and $\OUTS$ is the number of pairs reported.
\end{theorem}

\subsection{UNION}
\label{subsec:union}



We next consider the $(\tau,k)$-UNION-durable pairs under the cardinality constraint $k$ on the witness. This algorithm follows the same high-level idea as Section~\ref{subsec:sum}, but relies on a different primitive.

\paragraph{Primitive: Interval-$k$-UNION-Durability.} %
%The reporting algorithm for UNION-durable pairs shares the same high-level framework as that for SUM, except the data structure used for computing the {\em interval-UNION-durability} primitive:
%
%\begin{definition}[Interval-UNION-Durability]
%    Given a set of intervals $\mathcal{I}$, the goal is to construct a data structure such that for any interval $I'$, the aggregated durability $\displaystyle{\big|\bigcup_{I \in \mathcal{I}} (I\cap I')\big|}$ can be computed.
%\end{definition}
%\begin{itemize}
%    \item {\bf Compute-UNION-Durability.} Given a set of intervals $\mathcal{I}$, the goal is to construct a data structure for $\mathcal{I}$ such that given a query interval $I'$, the aggregated durability $|\bigcup_{I \in \mathcal{I}} I\cap I'|$ can be computed.
%\end{itemize}
%It turns out that a near-linear space data structure with $\polylog(n)$ query time is challenging. Hence, we focus on a simpler version by limited the number of intervals that contribute to the union. A pair of points $(p,q)$ is $\tau$-$k$-UNION-durable if $\dist(p, q)\leq 1$ and there exists a set of nodes $S \subseteq P$ with $|S|\leq k$ such that:
%%\begin{itemize}[leftmargin=*]
%    \item For every $q' \in S$, $\dist(p,q')\leq 1$, $\dist(q,q')\leq 1$;
%    \item $|I_p\cap I_q\cap (\bigcup_{s\in S}I_s)| \geq \tau$.
%\end{itemize} 
%The goal is to report all $(\tau,k)$-UNION-durable pairs for an arbitrary input parameter $k\ge 1$. 
%We introduce the following primitive query:
%
%\begin{definition}[Detect-$k$-UNION-Durability]
    Given a set of intervals $\mathcal{I}$, $\tau > 0$, and a positive integer $k$, the goal is to construct a data structure such that for any interval $I'$ and parameter $k$, whether there exists a subset of intervals $ U \subseteq \mathcal{I}$ such that $|U| \le k$ and $\big|\bigcup_{I \in \mathcal{I}} (I\cap I')\big| \ge \tau$, can be decided efficiently.
%
%\end{definition}
%\begin{itemize}
 %   \item {\bf Detect-UNION-Durability.} Given a set of intervals $\mathcal{I}$ and durability parameter $\tau > 0$, the goal is to construct a data structure such that, for any query interval $I'$ and parameter $k$, we check whether there exists a subset of intervals $ U \subseteq \mathcal{I}$ such that $|U| \le k$, and $|\bigcup_{I \in U} I\cap I'|\geq \tau$. 
%\end{itemize}

In particular, we find a set of intervals $U$ of size $k$ that maximizes $\big|\bigcup_{I \in \mathcal{I}} (I\cap I')\big|$. It is straightforward to relate this problem to the {\em maximum $k$-coverage} problem: given a family of sets over a set of elements, the goal is to choose $k$ sets to cover the maximum number of elements. The standard greedy algorithm gives an $(1-1/e)$-approximation for the maximum $k$-coverage problem~\cite{hochbaum1996approximating}. Back to our problem, each $I \in \I$ defines a new interval $I \cap I'$, and the goal is to choose $k$ intervals to cover the maximum region of $I'$. 


We describe some high-level idea here. Details on data structures, pseudocode, correctness and complexity analysis are given in Appendix~\ref{appendix:aggregate}. Let $U$ be the set of chosen intervals, which will cut $I'$ into a set of multiple uncovered sub-intervals of $I' - \bigcup_{I \in U} I$. Let $H$ store a set of interval pairs, say $(I,I'')$ indicating $I$ is not covered by any interval in $U$ and $I''$ is the non-chosen interval from $\mathcal{I} \setminus U$ that has the maximum intersection with $I$.
Each time, the greedy algorithm finds the interval covering maximum uncovered region of $I'$, by finding the pair in $H$ with maximum intersection, say $(I_x, I_y)$. After adding $I_y$ into $U$, it remains to remove $(I_x,I_y)$ from $H$, update the uncovered sub-intervals induced by $I_x - I_y$ (which is at most 2) as well as the corresponding pairs in $H$.

Using a modified interval tree of size $O(n\log^2 n)$, this greedy strategy runs in $O(k\log^2 n)$ time.
The overall algorithm of reporting $(\tau,k)$-UNION durable pairs is the same as Section~\ref{subsec:sum}. The only difference is the new primitive to execute the greedy algorithm efficiently.  In Appendix~\ref{appendix:aggregate}, we show that the number of pairs $\OUTU$ reported satisfies 
$|K_{\tau,k}| \leq \OUTU \leq |K_{(1-1/e)\tau, k}^{\eps}|$.

\begin{theorem}
    \label{thm:offlineUNION}
   Given a metric space $(P,\phi)$ of $n$ points, $\tau >0$, $\eps > 0$ and a positive integer $k$,
    the $\eps$-approximate \problemthree\ problem with UNION can be solved in $O(n\cdot\eps^{-O(\ddim)}k\log^2 n + \OUTU \cdot \eps^{-O(\ddim)}k\log^3 n)$ time, where $\ddim$ is the doubling dimension of $P$ and $\OUTU$ is the number of pairs reported.
\end{theorem}

==> intro.tex <==
\section{Introduction}

We start with two examples to motivate the problem of finding durable patterns in temporal proximity graphs.

\begin{example}
\label{exmpl:1}
Consider an online forum with social networking features, where users with similar profiles are connected as friends.
Each user may be active on the forum only for a period of time during the day. We are interested in finding cliques of connected users who are simultaneously active for a sufficiently long time window. Such queries are useful, for example, to forum administrators who want to understand how the social network influences interactions and leverage it to attract additional forum activities.
\end{example}

\begin{example}
\label{exmpl:2}
Consider a co-authorship graph where two researchers are connected if they have written at least one paper together. Further suppose that researchers are each associated with a time period where they remain active in research. Besides researchers with direct co-authorship, we might be interested in pairs who co-authored with a set of common researchers over a long period of time. For example, there might be two professors who have over the years collaborated with multiple students in common, even though these students may be research-active at different times.
\end{example}
%While there are many ways to define temporal graphs, in this paper, we consider temporal graphs where each node is associated with a time interval, which begins when the node is added to graph and ends when the node is deleted.

\change{
Social networks such as the graph in Example~\ref{exmpl:1} can be embedded in the space of user profiles, as proximity graphs with low intrinsic dimension~\cite{verbeek2014metric}.
From the co-authorship dblp graph~\cite{yang2012defining}, we use the authorship-relations (scientist $a$ has written paper $p$ with scientist $b$), to construct a ``frequency'' graph for Example~\ref{exmpl:2}. Two authors are connected if they have written at least $m$ papers together, for some $m\geq 1$.
This graph can also be embedded as a proximity graph, with low intrinsic dimension since it is sparse and ``nicely'' structured in the sense that vertices can be efficiently clustered or grouped based on their proximity to one another.
Generally, it is known that the graphs arising in many applications (e.g. social network, transportation network, Internet) can be approximated as \emph{proximity graphs}, where nodes are embedded as points in some high-dimensional space with small intrinsic dimension and nearby points are connected by an edge (or the distance between points approximates the shortest path between the corresponding nodes)~\cite{verbeek2014metric, zhao2010orion, zhao2011efficient}.
%For instance, the social network in Example~\ref{exmpl:1} is formed in the space of user profiles.

The problem of finding (durable) patterns in general graphs is hard: known (conditional) lower bounds suggest that it is unlikely to have near-linear algorithms~\cite{abboud2014popular, alon2008testing, patrascu2010towards}.
This observation raises the question whether computing durability patterns is easier in proximity graphs, for which we are not aware of any efficient algorithms. In this paper, we assume that the node embedding is given and the underlying graph is a proximity graph. We work with an implicit representation of the underlying proximity graph, i.e., we never construct the graph itself explicitly, and we design efficient algorithms whose running time depend on the intrinsic dimension (\emph{doubling dimension}) of the data. Our approach extends to a larger class of graphs (such as interval graphs, permutation graphs, and grid graphs).
%A challenging question, which is a good future direction and beyond the scope of this work, is whether we can extend our approach to design algorithms for finding durable patterns on general graphs, without first computing an embedding, which can run in near-linear time if the underlying graph happens to be a proximity graph.
}
Next, we formally define the problems we study. Our basic notation is summarized in Appendix~\ref{appndx:tableNotation}.

\subsection{Problem Definition}
Let $(P,\dist)$ be a metric space over a set of $n$ points $P\subset \Re^d$, for some $d\geq 1$, and a metric $\dist$.
\change{
The \emph{spread} of a set $P$ is defined as the ratio of the maximum and minimum pairwise distance in $P$. In most datasets arising in practice the spread is polynomially bounded.
}
For a parameter $r>0$, let $G_\dist(P,r)=(P,E)$ where $E=\{(p,q)
\mid \dist(p,q)\leq r\}$ be a {\em proximity graph}, also called a {\em unit--disk} graph.
For simplicity, we assume $r=1$ and let $G_\phi(P)=G_\phi(P,1)$.
Each point $p\in P$ is associated with a time interval $I_p=[I_p^-, I_p^+]$, noted as the {\em lifespan}, which indicates that $p$ is inserted at time-stamp $I_p^-$ and deleted at time-stamp $I_p^+$.%~\footnote{We note that there are many different ways to define temporal graphs. As shown in~\cite{hu2022computing}, the formulation of lifespan can capture many variants of other definitions and our algorithms can be applied correspondingly.}

%\change{
%For simplicity in this paper we assume that a metric space $(P,\phi)$ is defined over a set of $n$ point in $\Re^d$, where each point is associated with a lifespan, and a distance function $\phi$.}

%\change{Let $G$ be a graph. We assume that there exists an embedding where $G$ can be approximated as a proximity graph $G_\dist$. We are given an implicit representation $(P,\dist)$ of the underlying proximity graph $G_\dist$, where $P$ is the set of points/nodes in $G_\dist$, and $\dist(\cdot)$ is the distance function between the points/nodes in $G_\dist$. Our goal is to report durable patterns in $G_\dist$ working only with its implicit representation $(P,\dist)$. 
%Our algorithms for report (approximately) durable structures in $G$, use only the implicit representation $(P,\dist)$ without constructing the graph $G_\dist$.
%}

\paragraph{Doubling dimension.}
For $x\in \Re^d$ and $r\geq 0$, let $\mathcal{B}(x,r)=\{y\in \Re^d\mid \dist(x,y)\leq r\}$ be the ball (under the metric $\dist$) centered at point $x$ of radius $r$. 
A metric space $(P,\dist)$ has doubling dimension $\ddim$ if for any $p\in P$ and $r>0$, $\mathcal{B}(p,r) \cap P$ can be covered by the union of at most $2^\ddim$ balls of radius $r/2$.
For any $\alpha>0$, the metric space $(P,\ell_\alpha)$ has doubling dimension $d$ for any $P\subset\Re^d$, but for specific $P\subset\Re^d$ it can be much smaller (e.g. points lying on a $2$-dimensional plane or sphere has doubling dimension $2$).
\change{Doubling dimensions and their variants are popular approaches for measuring the intrinsic dimension of a data set in high dimension. See e.g.~\cite{DBLP:conf/iclr/PopeZAGG21, facco2017estimating, bshouty2009using, DBLP:conf/iclr/PopeZAGG21}. Because of this, many papers in ML, database systems, data mining, and theory analyze the running time in terms of doubling dimension.}


\paragraph{Durable triangles.}
%
Motivated by Example~\ref{exmpl:1}, we define {\em $\tau$-durable triangles} below.
A triplet $(p_1, p_2, p_3) \in P \times P \times P$ forms a {\em triangle} in $G_\dist(P)$ if $\dist(p_1, p_2)$, $\dist(p_2, p_3)$, $\dist(p_1,p_3)\le 1$. The {\em lifespan} of $(p_1, p_2, p_3)$ is defined as $I(p_1, p_2, p_3) = I_{p_1}\cap I_{p_2}\cap I_{p_3}$.
In the following, we also use a notion of $\eps$-approximate triangles for a parameter $\eps>0$.
A triplet $(p_1, p_2, p_3)$ forms an {\em $\eps$-approximate triangle}, or {\em $\eps$-triangle} for brevity, if $\dist(p_1, p_2)$, $\dist(p_2, p_3)$, $\dist(p_1,p_3)\leq 1+\eps$.  
%
For a durability parameter $\tau > 0$, $(p_1, p_2, p_3)$ is \emph{$\tau$-durable} if $I(p_1, p_2, p_3)\ge \tau$.
Let $T_{\tau}$ be the set of all $\tau$-durable triangles. Let also $T_{\tau}^{\eps}$ be the set of all $\tau$-durable $\eps$-triangles. Notice that $T_{\tau}\subseteq T_{\tau}^{\eps}$.

\vspace{0.5em}
\textbf{\textit{Problem 1: \problemone.}}  Given a metric space $(P,\dist)$ and $\tau \ge 0$, it asks to report all $\tau$-durable triangles in $G_\dist(P)$.
\vspace{0.5em}

\begin{comment}
\begin{definition}[\textbf{\problemone}] 
\label{def:offline}
    Suppose we are given a metric space $(P,\dist)$ and a durability parameter $\tau \ge 0$. It asks to report all $\tau$-durable triangles in $G_\dist(P)$.
\end{definition}
\end{comment}
 
%\change{As pointed out, social networks can be embedded as proximity graphs with low doubling dimension~\cite{verbeek2014metric}. 

\change{
Recall Example~\ref{exmpl:1}.
Social networks can be embedded as proximity graphs with low doubling dimension~\cite{verbeek2014metric}.
Each point $p_i$ represents a user and the goal is to find triplets (or generally cliques) of similar users who are simultaneously active on the forum. While each point has one interval, a user from Example~\ref{exmpl:1} might be active multiple times. We can extend the problem definition so that each point has at most $m$ intervals. The complexities of the algorithms we propose in the next sections increase by a factor of $m$.}

However, in many practical cases, we may not have a clear choice of the durability parameter in mind, and we may want to explore with different durability values. Supporting this mode of querying motivates
the problem of incrementally reporting $\tau$-durable triangles.
Here, queries arrive in an online fashion, each specifying a different durability parameter.
Instead of computing each
query from scratch, we want to leverage the previous query results and only incrementally compute what is new.

\vspace{0.5em}
\textbf{\textit{Problem 2: \problemtwo.}} Given a metric space $(P,\dist)$ and $\tau_1, \tau_2, \cdots$ arrive in an online fashion, for every $\tau_{i+1}$, it asks to report all $\tau_{i+1}$-durable triangles if $\tau_{i+1}>\tau_i$, and all $\tau_{i+1}$-durable but not $\tau_i$-durable triangles otherwise.
\vspace{0.5em}


Instead of computing the query results from scratch, we maintain the current results by leveraging the previous results.
More specifically, if $\tau_{i+1} > \tau_i$, $T_{\tau_{i+1}} \subseteq T_{\tau_i}$ since every $\tau_{i+1}$-durable triangle must also be $\tau_i$-durable.
On the other hand, if $\tau_{i+1} \le \tau_i$, $T_{\tau_{i+1}} \supseteq T_{\tau_i}$;
in this case it suffices to report triangles in $T_{\tau_{i+1}} - T_{\tau_i}$, i.e. those are $\tau_{i+1}$-durable but not $\tau_i$-durable, which together with $T_{\tau_i}$ would give $T_{\tau_{i+1}}$. Hence, we can incrementally build $T_{\tau_{i+1}}$ based on $T_{\tau_i}$.

\paragraph{Aggregated-Durable Pairs.}
%
Motivated by Example~\ref{exmpl:2}, we further investigate the notion of {\em aggregated durability} over triangles in temporal graphs. We consider two natural ways of aggregating durability -- \SUM\ and \UNION. For a pair $(p_1,p_2) \in P \times P$, and a subset of points $U \subseteq P$, the aggregated durability of $(p_1,p_2)$ with respect to $U$, is defined as 
$\textsf{AGG}(p_1,p_2,U) = \sum_{u\in U} \big|I(u, {p_1} ,{p_2})\big|$ for \SUM, and $\textsf{AGG}(p_1,p_2,U) = \big|\bigcup_{u\in U} I(u, {p_1} ,{p_2})\big|$ for \UNION. 
For a durability parameter $\tau > 0$, a pair $(p_1, p_2)\in P \times P$ is {\em $\tau$-aggregate--durable} if $\dist(p_1, p_2)\leq 1$, and there exists a subset of points $U \subseteq P$ such that (\romannumeral 1) $\dist(p_1,u), \dist(p_2, u) \le 1$ for any point $u \in U$ and (\romannumeral 2) $\textsf{AGG}(p_1,p_2,U) \ge \tau$. We also denote $U$ as the {\em witness} of $(p_1, p_2)$.  



\vspace{0.5em}
\textbf{\textit{Problem 3: \textbf{\problemthree.}}}  Given a metric space $(P,\dist)$ and $\tau \ge 0$, it asks to report all $\tau$-aggregate-durable pairs in $G_\dist(P)$.
\vspace{0.5em}

\change{
Recall Example~\ref{exmpl:2}. As pointed out, the frequency graph constructed from the co-authorship dblp graph, can be embedded as a proximity graph with low doubling dimension (e.g., 12~\cite{linkDdim}).
Each point $p_i$ represents a researcher, and the goal is to find the pairs of researchers $p_i, p_j$ that collaborated sufficiently with various others in terms of total time over all collaborators (\SUM), or over a large portion of $(p_i, p_j)$'s common lifespan (\UNION).}

\begin{table}[t]
    \centering
    \begin{tabular}{c|c}
     \toprule
    Problems & Time Complexity $\O(\cdot)$\tablefootnote{$\O(\cdot)$ hides a $\polylog n$ factor. The hidden constants in $O(\cdot)$ and $\O(\cdot)$ notation may depend on $\rho$, which is assumed to be a constant.} \\\hline
    \problemone & $n\eps^{-O(\ddim)}+\OUTOFF$\\\hline
    \problemtwo & $\eps^{-O(\ddim)} \cdot \OUTON$\\\hline
    \problemthree--\SUM\ & $n\eps^{-O(\ddim)}+\eps^{-O(\ddim)} \cdot \OUTS$  \\\hline
    \problemthree--\UNION\ & $nk\eps^{-O(\ddim)}+k\eps^{-O(\ddim)} \cdot \OUTU$  \\
    \bottomrule
    \end{tabular}
    \vspace{1em}
    \caption{Summary of our main results skipping $\polylog n$ factors. $n$ is the input size, i.e., the number of nodes in the graph. $\tau$ is the durability parameter. $\OUT_X$ is the output size for each different version of the problem. $\eps$ is the approximation ratio. $k$ is the parameter used for $(\tau,k)$-\UNION\ durability.
    }
    \vspace{-1em}
    \label{table:results}
\end{table}

As we will see later, computing $\textsf{AGG}(p_1,p_2,U)$ for the \UNION\ is very challenging due to the inherent hardness of computing the union of intervals that intersect a query interval. Instead, we consider a restricted version of $\tau$-\UNION-durable pairs, with cardinality constraint on the witness. For a durability parameter $\tau$ and a positive integer $k \in \mathbb{Z^+}$, a pair $(p_1, p_2) \in P \times P$ is {\em $(\tau,k)$-\UNION-durable} if $(p_1,p_2) \in E$ and there exists a subset of points $U \subseteq P$ such that (\romannumeral 1) $(p_1,u)$, $(p_2,u)\in E$ for any point $u\in U$; (\romannumeral 2) \textsf{AGG}$(p_1, p_2, U) \ge \tau$; (\romannumeral 3) $|U| \le k$. For simplicity, we denote $K_{\tau}$ as the set of $\tau$-\SUM\ durable pairs, and $K_{\tau,k}$ as the set of $(\tau,k)$-\UNION\ durable pairs.
We also mention aggregate-durable pairs defined on $\eps$-triangles. 
A pair $(p,q) \in P\times P$ is a {\em $\tau$-aggregate-durable $\eps$-pair} if all corresponding durability conditions for $\tau$-aggregate-durable pairs change from $1$ to $1+\eps$. Let $K_{\tau}^\eps$ be the set of $\tau$-\SUM\ durable $\eps$-pairs, and $K_{\tau, k}^\eps$ be the set of $(\tau,k)$-\UNION\ durable $\eps$-pairs.

\subsection{Our Results and Approach}
\change{
\smallskip \noindent {\bf Our Results.} We present algorithms for \emph{$\eps$-approximate} versions of Problems 1--3, as summarized in Table~\ref{table:results}. In all cases we report all durable triangles along with some durable $\eps$-triangles.
The running time is always near-linear in terms of the input and output size, which is almost the best one could hope for.

We assume that $P$ has polynomially bounded spread.
Our algorithms work for unbounded spread -- a $\log n$ factor in the running time gets replaced by $\log \Delta$, where $\Delta$ is the spread, or one can sometimes use a more sophisticated data structure to replace the $\log \Delta$ factor with $\log n$ even for unbounded spread. Furthermore, the spread in real datasets is indeed polynomially bounded -- and as such a common assumption in machine learning and data analysis.

We also assume $\ddim$ to be a constant, i.e., $(P,\dist)$ has bounded doubling dimension.
Our algorithms work for data in any doubling dimension $\ddim$. It is only the time complexity that depends on $\ddim$. It has been widely shown that graphs arising in practice have low doubling dimension~\cite{ng2002predicting, tenenbaum2000global, feldmann2020parameterized, damian2006distributed, zhoudoubling, verbeek2014metric}.
Empirical studies in these papers and other sources (e.g., \cite{linkDdim}) show that the doubling dimension of router graphs, internet latency graphs, citation graphs, and movie database graphs are 14, 9, 12, and 14 respectively.
In our work, we assume the doubling dimension to be a small constant and the provable bound on the running time depends exponentially in $\ddim$, as is usually the case; 
in practice the dependency on doubling dimension could be much smaller depending on the data set.

{\bf (Section~\ref{sec:offline})} For \problemone, we present an $\O(n\eps^{-O(\ddim)}+\OUTOFF)$-time algorithm, where $\OUTOFF \in [|T_{\tau}|,|T_{\tau}^\eps|]$.
Moreover, for the $\ell_\infty$ metric, this result can be improved to $\O(n+|T_\tau|)$. Our data structures can be extended to support delay-guaranteed enumeration, and support dynamic settings where nodes in the proximity graph can be inserted or deleted according to their lifespan. 

{\bf(Section~\ref{sec:online})} For \problemtwo, we construct a size-$\O(n)$ data structure in $\O(n)$ time, such that if $\tau_{i+1}<\tau_i$, (i.e. $\tau_{i}$ is the durability parameter of the previous query), the delta results are reported in $\O(\eps^{-O(\ddim)}\cdot \OUTON)$ time, where $\OUTON \in \left[|T_{\tau_{i+1}} - T_{\tau_{i}}|, |T_{\tau_{i+1}}^\eps -T_{\tau_{i}}^\eps|\right]$ is the output size, and if $\tau_{i+1}\geq \tau_i$, we report the $\tau_{i+1}$-durable triangles in time $\O(\eps^{-O(\ddim)}\cdot \OUTON)$ time, where $\OUTON \in \left[|T_{\tau_{i+1}}|, |T_{\tau_{i+1}}^\eps|\right]$.
For the $\ell_\infty$ metric, the \problemtwo\ problem can be solved exactly in $\O(|T_{\tau_{i+1}}\setminus T_{\tau_i}|)$ time.

 {\bf (Section~\ref{sec:aggregate})} For \problemthree\ with \SUM\ function, we present an $\O(n\eps^{-O(\ddim)}+ \OUTS \cdot\eps^{-O(\ddim)})$-time algorithm, where $\OUTS \in \left[K_\tau, K^\epsilon_\tau\right]$, is the output size. For \problemthree\ with $(\tau,k)$-\UNION, we present an $\O(n k\eps^{-O(\ddim)}+ \OUTU \cdot k\eps^{-O(\ddim)})$-time algorithm, where $\OUTU \in \left[|K_{\tau, k}|, \big|K_{(1-1/e)\tau, k}^{\eps}\big|\right]$.
 %It also implies an $\O\left(n^2\eps^{-O(\ddim)} + \OUT \cdot n\eps^{-O(\ddim)}\right)$-time algorithm for the \problemthree\ with \UNION.

\noindent {\bf Our approach.} To obtain these results, our main approach is to construct a hierarchical space decomposition that consists of a canonical set of balls, using a \emph{cover tree}. We use the canonical set of balls to obtain a compact implicit representation of points within distance $1$ from each point $p \in P$, and then use an {\em interval tree} along with auxiliary data structures to report durable triangles in linear time.
%All data structures used will be described later.
When it comes to the online setting, we additionally maintain an activation threshold for each point with respect to different durability parameters. More specifically, for each durability parameter $\tau$, we design an oracle that can efficiently find the largest value $\tau' <\tau$ such that $p$ participates in a $\tau$-durable triangle that is not $\tau'$-durable, which is key to achieve near-linear time complexity.  
To find aggregate-durable pairs, we built auxiliary data structures to compute the sum or union of intervals intersecting any given interval. Additionally, we identify a special ordering of $P$, such that only a bounded number of pairs that are not aggregate-durable will be visited, hence the linear-time complexity can be guaranteed.
}

\paragraph{Implications.} \change{
%Firstly, our proposed solution can be extended to the settings where each point is associated with a set of disjoint intervals, which arise when the same point can be inserted and deleted multiple times. The complexity of our algorithm only increases by a factor of $m$, where $m$ is the number of disjoint intervals. 
%
Although we focus on the $\eps$-approximate version of all problem, we can handle the exact version returning only the real durable patterns in all cases. Each time a triplet $(p,q,s)$ is found, we check in $O(1)$ time if $\dist(p,q), \dist(p,s), \dist(q,s)\leq 1$, and only report it if satisfied. The total running time does not increase asymptotically.

Our algorithms also work for any $\ell_\alpha$-norm metric\footnote{If $\dist$ is the $\ell_\alpha$ norm then $\dist(p,q)=\left(\sum_{j=1}^d|p_j-q_j|^\alpha\right)^{1/\alpha}$, where $p_j, q_j$ are the $j$-th coordinates of points $p$ and $q$, respectively.} or metric with bounded expansion constant\footnote{A metric space $(P,\dist)$ has expansion constant $D$ if $D$ is the smallest value such that for any $p\in P$ and $r>0$ $|P\cap \mathcal{B}(p,2r)|\leq D\cdot|P\cap \mathcal{B}(p,r)|$, where $\mathcal{B}(p,r)$ is the ball with center $p$ and radius $r$.}, with roughly the same complexity. Moreover, all our results for reporting triangles can be straightforwardly extended to reporting cliques of constant size, paths of constant size, and star patterns. See details in Appendix~\ref{appndx:extensions}.
}

==> offline.tex <==
\section{Reporting Durable Triangles}
\label{sec:offline}

\begin{figure}
    \centering
    \includegraphics[scale=0.2]{img/offlineddim.png}
    \caption{An illustration of Algorithm~\ref{alg:offline-2}: $p$ is visited. The small (possibly overlapping) balls are the balls representing the canonical subsets of the cover tree. Each point within distance $1$ from $p$ lies in exactly one canonical node/ball. We report the triangles formed by $p$ and the points in red and blue canonical balls that satisfy the durability constraint. We do not report triangles formed by $p$ and the points in blue and green canonical balls.}
    \label{fig:offline-2}
\end{figure}

In this section, we describe a near-linear algorithm for the $\eps$-approximate \problemone\ problem. As mentioned, we describe the algorithm for any general metric with constant doubling dimension. In Appendix~\ref{appndx:linfty}, we show how to solve the problem exactly for $\ell_\infty$ metric.

\mparagraph{High-level Idea}
We visit each point $p\in P$ and report all $\tau$-durable triangles $p,q,s$ that $p$ participates in with $I_p^-\geq \max\{I_q^-,I_s^-\}$. We run a $\tau$-durable ball query ($\DTC$) around $p$ and get an implicit representation (consisting of a bounded number of canonical subsets) of all points within distance $1$ from $p$ while $I_p^-$ is the largest left endpoint of their temporal intervals. Recall that each canonical subset in $\DTC$ consists of points within a ball of a small enough radius, so it is safe to consider that all points in the ball lie at its center.
For every pair of canonical subsets/balls, if the distance between them is bounded by $1+\eps/2$, we report all $\tau$-durable triangles consisting of $p$ and the Cartesian product of the points in the pair.


\begin{algorithm}[t]
\caption{{\sc ReportTriangle}$(p, \tau, \epsilon, \DTC)$}
\label{alg:offline-2}

$\C_{p} \gets \DTCQ(p,\tau,\eps/2)$\;
Assume $\C_{p} = \{\C_{p,1}, \C_{p,2}, \cdots, \C_{p,k}\}$\;
\ForEach{$j \in [k]$}{
    Report $(p,q,s)$ for $(q,s) \in \mathcal{C}_{p,j} \times \mathcal{C}_{p,j}$ if $q \neq s$\;
}
\ForEach{$(i,j) \in [k] \times [k]$ with $i < j$}{
        \If{$\dist(\textsf{rep}_i, \textsf{rep}_j) \le 1 + \frac{\epsilon}{2}$}{
        Report $(p,q,s)$ for every $q \in \C_{p,i}$ and $s \in \C_{p,j}$\;
            
        }
    
    }

\end{algorithm}


%For general metrics, we adopt similar high-level framework by enumerating the $\tau$-durable triangles participated by each point. When we had points in $\Re^d$, we used a range tree to get an implicit representation of points within distance $1$ from a point $p$. If the doubling dimension (or expansion constant) is bounded we can use the cover tree (as described in Section~\ref{subsec:structures}) to get approximately an implicit representation of points within distance $1$ from $p$. Recall that $P$ is a set of points, where each point $p$ is associated with the lifespan interval $I_p$. 

\paragraph{Algorithm.}
Our algorithm is described in Algorithm~\ref{alg:offline-2}.
As the preprocessing step, we construct the data structure $\DTC$ as described in Section~\ref{sec:tau-durable-ball} over $P$. Let $p$ be a point visited. We run a $\tau$-durable ball query $\DTCQ(p,\tau,\eps/2)$\footnote{We define $\DTCQ(p,\tau,\eps/2)$ and not $\DTCQ(p,\tau,\eps)$ as in Section~\ref{sec:preliminary} for technical reasons.} and obtain a canonical set of nodes $\mathcal{C}_p=\{\C_{p,1}, \C_{p,2}, \ldots, \C_{p,k}\}$ for $k = O(\eps^{-\ddim})$ (see also Figure~\ref{fig:offline-2}). Each $\C_{p,j}$ represents a node in the cover tree of $\DTC$ with diameter $\eps/2$.
For each such node $\C_{p,j}$ we get $O(\log n)$ canonical subsets of the points $P_{(p,j,\tau)}=\{p'\in P\cap \C_{p,j}\mid I_{p'}^+\geq I_p^-+\tau, I_{p'}^-\leq I_p^-\}$, i.e., the points in $C_{p,j}$ whose intervals sufficiently intersect $I_p$, running a query in the interval tree stored at $\C_{p,j}$, as explained in Section~\ref{sec:tau-durable-ball}.
With a slight abuse of notation, we often use $\C_{p,j}$ to denote $P_{(p,j,\tau)}$. Moreover, let $\textsf{rep}_j$ be the representative point of the node $\C_{p,j}$.
Similarly, we further distinguish a $\tau$-durable triangle $(p,q,s)$ into two types: (1) $q,s \in \C_{p,j}$; (2) $q \in \C_{p,i}$, $s\in \C_{p,j}$ for $i \neq j$. We only need to report triangles in type (1) when $|\C_{p,j}| >1$, i.e., there are multiple points from $\C_{p,j}$ within durability threshold, hence every pair $(q,s) \in \C_{p,j} \times \C_{p,j}$ with $q \neq s$ must form a $\tau$-durable triangle with $p$. To report triangle in type (2), we check for every pair $\C_{p,i}, \C_{p,j}$ with $i \neq j$: if $\dist(\textsf{rep}_i, \textsf{rep}_j)\leq 1+\eps/2$, which implies $\dist(q,s) \le 1+ \eps$ for any point $q \in \C_{p,i}$ and $s \in \C_{p,j}$, we report the Cartesian product of $\C_{p,i} \times \C_{p,j}$, which is exactly the set of pairs that form a $\tau$-durable triangle in type (2) with $p$. 

\mparagraph{Correctness}
For any triangle $(p,q,s)$ reported, we note that $\dist(p,q) \leq 1+\eps,\dist(p,s) \leq 1+\eps, \dist(q,s)\leq 1+\eps$ and $|I_p\cap I_q\cap I_s|\geq \tau$. %Hence, we don't report any $\tau$-durable triangle
%\begin{itemize}
%    \item $\dist(p,q),\dist(p,s), \dist(q,s)\leq 1+\eps$;
%%    \item $|I_p\cap I_q\cap I_s|\geq \tau$
%\end{itemize}
%Hence, we do not return any $(\tau,x)$-durable triangle for any $x>1+\eps$. 
We only report a triangle $(p,q,s)$ when we search over the neighborhood of the newest point ($I_p^-\geq \max\{I_q^-,I_{s}^-\}$) so it is straightforward to observe that every triangle is reported once. Then, it remains to show that every $\tau$-durable triangle must be reported. Consider an arbitrary $\tau$-durable triangle $(p,q,s)$. W.l.o.g, assume $I_p^-\geq I_q^-$ and $I_p^-\geq I_s^-$. When $p$ is visited, it follows from the definition of $\DTCQ(p,\tau,\eps/2)$, that $q\in \C_{p,i}$ and $s \in \C_{p,j}$. If $i=j$, then $|\C_{p,i}|\geq 2$, so $(p,q,s)$ must be reported by line 4. If $i\neq j$, we have $\dist(\textsf{rep}_i,\textsf{rep}_j)\leq \dist(\textsf{rep}_i,q)+\dist(q,s)+\dist(s,\textsf{rep}_j) \leq \eps/4+1+\eps/4\leq 1+\eps/2.$
In that case, $(p,q,s)$ must be reported by line 7 of Algorithm~\ref{alg:offline-2}. 

\mparagraph{Time Complexity} Implied by Lemma~\ref{lem:helper-2}, $\DTC$ can be constructed in $O(n\log^2 n)$ time.
For each point $p \in P$, we run a $\tau$-durable ball query on $\DTC$ in $O(\eps^{-O(\ddim)}\log n)$ time. Moreover,  $|\mathcal{C}_p|=O(\eps^{-O(\ddim)})$. We also check all pairs of nodes in $\mathcal{C}$ to search for $\tau$-durable triangles in type (2), which takes additional $O(\eps^{-2\cdot O(\ddim)})$ time. As each $\tau$-durable triangle will be reported by Algorithm~\ref{alg:offline-2}, as well as some $\tau$-durable $\eps$-triangles, %might also be reported, due to the approximation. Thus, the number of triangle reported falls into the range $[|T_\tau|, |T^{1+\epsilon}_\tau|]$, where $T^{1+\epsilon}_\tau$ is set of $(\tau,1+\epsilon)$-durable triangles in the input graph. Thus, the time complexity of Algorithm~\ref{alg:offline-2} is bounded by $O(n(\eps^{-\ddim}\log n + \eps^{-2\cdot \ddim}+\log^2 n) + T^{1+\eps}_{\tau})$. 
hence $|T_{\tau}|\leq \OUTOFF \leq |T_{\tau}^\eps|$.
%$(p,q,s)$if it is $\tau,1)$-durable, by checking it in constant time each find we find a new triangle. So we can report only the $(\tau,1)$-durable triangles in the same running time.

\begin{theorem}
    \label{thm:offline-gen}
    Given a metric space $(P,\phi)$ of $n$ points, $\tau > 0$ and $\eps>0$, the $\eps$-approximate \problemone\ problem can be solved in 
    $O\left(n(\eps^{-O(\ddim)}\log n + \log^2 n) + \OUTOFF\right)$ time, 
    where $\ddim$ is the doubling dimension of $P$ and $\OUTOFF$ is the number of triangles reported.
\end{theorem}

\smallskip \noindent {\bf Remark 1.} For any $\ell_\alpha$ norm in $\Re^d$, we can simplify the data structure $\DTC$ using a quadtree instead of a cover tree. The running time and the approximation with respect to the overall number of triangles we visit remain the same.

\smallskip \noindent {\bf Remark 2.} \change{Our algorithm can be extended to support delay-guaran-teed enumeration of durable patterns, i.e., the time between reporting two consecutive patterns is bounded. After $O(n(\eps^{-O(\ddim)}\log n + \log^2 n))$ preprocessing time, we support $O(\eps^{-O(\ddim)}\log n)$-delay enumeration for the $\eps$-approximate \problemone\ problem.}

\smallskip \noindent {\bf Remark 3.} \change{Using a dynamic cover tree, our algorithm can be extended to the dynamic setting where we do not know all nodes upfront. In particular, if nodes are inserted or deleted according to their lifetime, we support amortized update time $O(\log^3 n)$. After the insertion of a node $p$, we report the new (if any) triangles that $p$ participates in (these are the triangles reported by Algorithm~\ref{alg:offline-2}), in time near linear to the number of newly reported triangles. We show the details in Appendix~\ref{appndx:dynamic}.}


==> online.tex <==
\section{Maintaining Durable Triangles}
\label{sec:online}

We next consider maintaining durable triangle when queries come in an online fashion.
We start by giving the intuition of our techniques in Section~\ref{sec:preprocessing} and move to the details for any metric space in Section~\ref{sec:ddim-reporting}. We handle the $\ell_\infty$-metric in Appendix~\ref{sec:linfty-reporting}.

\subsection{Activation Threshold}
\label{sec:preprocessing}

\noindent{\bf High-level Idea.} Assume that we have already reported the $\tau_i$-durable triangles as described in the previous section. For each point $p\in P$ that participates in at least one such triangle we need to have a method that computes what is the largest parameter $\tau'$ such that $\tau'<\tau_i$, and $p$ belongs to a $\tau'$-durable triangle that is not $\tau_i$-durable.
Assume that we knew the largest parameter $\tau'$ which we denote it with $\beta_p^{\tau_i}$.
Given the next durability parameter $\tau_{i+1}<\tau_i$, we could visit all points $p\subseteq P$ with $\tau_{i+1}\leq \beta_p^{\tau_i}\leq \tau_i$
and report all $\tau_{i+1}$-durable triangles formed by $p$ that are not $\tau_i$-durable.
In order to handle points $p$ that did not belong to any $\tau_i$ durable triangle in the previous iteration, we also store and maintain a set (implemented as a search binary tree) of points that have not been activated before. For each of these points $p$, we store what is the largest durability $\tau$ so that $p$ belongs to a $\tau$-durable triangle.
When $p$ is activated, we report all $\tau$-durable triangles that $p$ participates in as the newest point with respect to their time intervals.

\paragraph{Activation Threshold.} Below, we mostly describe how we can update $\beta_p^\tau$ efficiently and how we can report only triangles that are $\tau_{i+1}$-durable but not $\tau_i$-durable. We start by giving a more formal description of the activation threshold:

\begin{definition}[Activation threshold]
\label{def:delta}
    Given metric space $(P,\dist)$ and a durability parameter $\tau > 0$, the {\em activation threshold} of point $p \in P$ with respect to $\tau$ is defined as: 
    \[\beta^{\tau}_p = \max\{\tau' < \tau: \exists q,q', s.t., I_p^-\geq I_q^-, I_p^-\geq I_{q'}^-, \textrm{ and } (p,q,q') \textrm{ is a }\]
    \[\quad\quad\quad\quad\quad\quad\quad\textrm{$\tau'$-durable triangle but not a $\tau$-durable triangle}\}\]
    In the special case with $\tau = +\infty$, we denote $\alpha_p = \beta^{+\infty}_p$.
\end{definition}


\begin{lemma}
    For any $p \in P$, if $\tau < {\tau_{i}}$ and $\beta^{\tau_{i}}_p < \tau$, then $\beta^{\tau_{i}}_p = \beta^\tau_p$.
\end{lemma}


If there exists no pair of $(q,q')$ that $(p,q,q')$ is a triangle, we set the corresponding threshold to $-\infty$.
For simplicity, we use the notation $P_\tau\subseteq P$ to denote the set of points that are become active when the durability parameter is $\tau$.
We build a dynamic binary search tree $\mathcal{S}_\alpha$ for the points in $P$ with respect to $\alpha_p$. Moreover, we also build a dynamic binary search tree $\mathcal{S}_\beta$ for the points
that have been activated at least once.
Initially, we set $\mathcal{S}_\beta = \emptyset$. After computing $\alpha_p$ for every point $p \in P$, we can initialize $\S_\alpha$. Note that $\S_\alpha$ built for all input points stay unchanged, while $\S_\beta$ built for points only in $P_\tau$ will keep being updated, with the change of $\tau$.

Below, we focus on how to compute $\beta^\tau_p$. The high-level idea is to run a binary search on the domain of all possible durability parameters, until we find the largest one that satisfies the criteria. In particular, for each guess $\tau'$ of $\beta^\tau_p$ made by the search procedure, we need an efficient primitive (to be discussed later) for checking whether $p$ participates in any $\tau'$-durable but not $\tau$-durable triangle. It remains to identify the search space of activation thresholds for $p$. We observe that the lifespan of any triangle $(p,q,q')$ must be either $[I^-_p, I^+_{q}]$ or $[I^-_p, I^+_{q'}]$, thus the durability of any triangle that contains $p$ must fall into 
$\left\{I^+_{q} - I^-_p:q \in P, I^+_{q} \ge I^-_p\right\}$.  
Hence, it suffices to run a binary search over the right endpoints of intervals of the points in $P$, which has size $O(n)$. Next, we focus on how to check if a given point $p$ participates in any $\tau'$-durable but not $\tau$-durable triangle.

\paragraph{Data Structure.}
We construct the data structure $\DTCE$ as described in Section~\ref{sec:tau-durable-ball}. Its size is $(n\log^2 n)$, and it can be constructed in $O(n\log^3 n)$ time.
We note that in general metric spaces, we cannot compute $\beta^\tau_p$ exactly because $\DTCE$ does not find a family of canonical subsets only for the points within distance $1$ from $p$. Recall that we get an $\eps$-approximation.
Hence, we might activate a point for a $\tau_{i+1}$-durable $\eps$-triangle. This is not an issue as long as the new triangle was not reported in the previous iteration.

\subsection{Dynamic Algorithm}
\label{sec:ddim-reporting}
\noindent {\bf Compute Activation Thresholds.} For a set $P$ of $n$ points, we first build the data structure $\DTCE$ as described in Section~\ref{sec:tau-durable-ball} over $P$, and then invoke Algorithm~\ref{alg:offline-2}.
Recall that $\DTCE$ is the extended version of $\DTC$, to handle interval queries with one additional linear constraint on the intervals' endpoints as we will see later.
\begin{algorithm}[t]
\caption{{\sc DetectTriangle}$(p,\eps, \DTCE, \tau, \tau')$}
\label{alg:detect-general}

$\C_{p} \gets \DTCEQ(p,\tau,\tau',\eps/2)$\;
Assume $\C_{p} = \{\C_{p,1}, \C_{p,2}, \cdots, \C_{p,k}\}$\;
\ForEach{$j \in [k]$}{
   $\Lambda_j^p = 
    \left\{q \in \C_{p,j}: I^-_q \le I_p^-, I_p^- + \tau' \le I^+_q < I_p^- +\tau \right\}$\;
    $\Psi_j^p = \left\{q \in \C_{p,j}: I_q^-\leq I_p^-, I_q^+\geq I_p^-+ \tau \right\}$\;
    \lIf{$|\mathcal{C}_{p,j}| \ge 2$ and $|\Lambda_j^p|\geq 1$}{\Return \textbf{true}}
}
\ForEach{$(h,j) \in [k] \times [k]$ with $h < j$}{
        \If{$\dist(\textsf{rep}_h, \textsf{rep}_j) \le 1 + \frac{\epsilon}{2}$ and $|\C_{p,h}|\ge 1$ and $|\C_{p,j}| \ge 1$ and $|\Lambda_h^p\cup \Lambda_j^p|\geq 1$}{
            \Return \textbf{true}\;
        }
    
    }
\Return \textbf{false}\;
\end{algorithm}


As described in Algorithm~\ref{alg:detect-general}, we run $\DTCEQ(p, \tau, \tau', \eps/2)$ and get a family of $k=O(\eps^{-O(\ddim)})$ canonical subsets $\C_p=\{\C_{p,1},\ldots, \C_{p,k}\}$, which are the canonical nodes of the cover tree included in $\DTCE$.
For each $\C_{p,j}\in \C_p$ we use the interval tree in this node to further partition $\C_{p,j}$ into two non-intersecting subsets of points $\Lambda_j^p$ and $\Psi_j^p$.
Intuitively, for any point $q$ returned from $\C_{p,j}$, $\tau' \le |I_q \cap I_p| < \tau$ if $q \in \Lambda_j^p$, and $|I_q \cap I_p| \ge \tau$ otherwise. We note that we do not explicitly construct $\Lambda_j^p$ and $\Psi_j^p$. Instead, we find $O(\log^2 n)$ canonical subsets that contain all points in $\Lambda_j^p$ and $\Psi_j^p$ of each $j$, using $\DTCE$.
We slightly abuse the notation and we set $\C_{p,j}=\Lambda_j^p \cup \Psi_j^p$.
If there is a subset $C_{p,j}$ with cardinality at least $2$ that contains at least one point from $\Lambda_j^p$ then we return that there exists a $\tau'$-durable triangle that is not $\tau$-durable. Next, we check any pair of non-empty canonical subsets $C_{p,j}, C_{p,h}$ such that $\dist(\rep_j,\rep_h)\leq 1+\eps/2$ and if there exist at least one point in $\Lambda_j^p\cup \Lambda_h^p$ we return that there exists a $\tau'$-durable triangle that is not $\tau$-durable. In any other case we return that there is no new $\tau'$ durable triangle.
\begin{figure}
    \centering
    \includegraphics[scale=0.8]{img/update.pdf}
    \caption{An illustration of $\Lambda^p_j$ and $\Psi^p_j$. Assume $q_1,q_2 \in C_{p,j}$. Here, $q_1 \in \Lambda^p_j$ and $q_2 \in \Psi^p_j$.}
    \label{fig:updateddim}
\end{figure}
See Figure~\ref{fig:updateddim}. As mentioned, we perform at most $O(\log n)$ guesses and it takes $O(\eps^{-O(\ddim)}\log^2 n)$ time to run Algorithm~\ref{alg:detect-general} for each guess of $\tau'$.

\begin{algorithm}[t]
\caption{{\sc ReportDeltaTriangle}$(p,  \epsilon, \DTCE, {\tau_{i}}, \tau_{i+1})$}
\label{alg:report-delta-general}


$\C_{p} \gets \DTCEQ(p,\tau_{i},\tau_{i+1}, \eps/2)$\;
Assume $\C_{p} = \{\C_{p,1}, \C_{p,2}, \cdots, \C_{p,k}\}$\;
\ForEach{$j \in [k]$}{
    $\Lambda_j^p = 
    \left\{q \in \C_{p,j}: I^-_q \le I_p^-, I_p^- + \tau_{i+1} \le I^+_q < I_p^- +{\tau_{i}}\right\}$\;
    $\Psi_j^p = \left\{q \in \C_{p,j}: I_q^-\leq I_p^-, I_q^+\geq I_p^-+{\tau_{i}} \right\}$\;
    Report $(p,q,q')$ for $(q,q') \in \Lambda^p_{j} \times  \Lambda^{p}_j$ if $q \neq q'$\;
    Report $(p,q,q')$ for $q \in \Lambda^p_{j}$ and $q'\in \Psi^{p}_j$ if $q \neq q'$\;
}
\ForEach{$(h,j) \in [k] \times [k]$ with $h < j$}{
        \If{$\dist(\textsf{rep}_h, \textsf{rep}_j) \le 1 + \frac{\epsilon}{2}$}{
        Report $(p,q,q')$ for every $(q,q')\in \Lambda^{p}_h\times \Psi^p_j$, $(q,q')\in \Psi^p_h\times \Lambda^p_j$, and $(q,q')\in \Lambda^p_h \times \Lambda^p_j$ \;
        }
    
    }
\end{algorithm}

 
 The high-level idea of our algorithm is to search over $\mathcal{S}_\alpha, \mathcal{S}_\beta$ to find all points that belong to a $\tau_{i+1}$-durable triangle (or $\eps$-triangle) that is not $\tau_i$-durable. For each such point $p$, we report all $\tau$-durable triangles such that i) $p$ participates in this triangle, the triangle is not a $\tau_i$ durable $\eps$-triangle, and iii) $p$ is the newest point among the points of the triangle. The actual reporting algorithm is a simple modification of Algorithm~\ref{alg:detect-general} for detecting a triangle.
 
 \mparagraph{Update and Report} Suppose $\tau_{i+1}, \tau_i$ are the durability parameters of current and last query separately. For completeness, we set $\tau_0 = -\infty$. We distinguish the following two cases.
 
 \mparagraph{Case 1: $\tau_{i+1} > \tau_i$}  Set $\mathcal{S}_\beta=\emptyset$. We simply issue a range query to $\mathcal{S}_\alpha$ to find the set of points $P_{\tau_{i+1}}\subseteq P$ that participates in at least one $\tau_{i+1}$-durable triangle, and then invoke Algorithm~\ref{alg:offline-2} for each point $p\in P_{\tau_{i+1}}$. Additionally, we reconstruct  $\S_\beta$ from scratch, by adding every point $p \in P_{\tau_{i+1}}$ into $\S_\beta$ with the value of $\beta^\tau_p$. 
 If $\OUTON$ is the output size in {\bf Case 1}, we have $|T_{\tau_{i+1}}|\leq \OUTON\leq |T_{\tau_{i+1}^\eps}|$.
 
 \mparagraph{Case 2: $\tau_{i+1} < \tau_i$}
 Recall that our target is to report all triangles in $T_{\tau_{i+1}} \setminus T_{\tau_i}^\eps$. We first point out that any triangle in $T_{\tau_{i+1}} \setminus T_{\tau_i}$ falls into one of the following two cases: there exists one point, say $p$, with {\bf Case (2.1)} $\tau_{i+1} \leq \alpha_p < \tau_{i}$, or {\bf Case (2.2)} $\tau_{i+1} \le \beta^{\tau_{i}}_p < \tau_i < \alpha_p$.

 
 \mparagraph{Case (2.1)} We find all points $p$ with $\tau_{i+1} \leq \alpha_p < \tau_i$ from $\mathcal{S}_\alpha$. Let $P_{\tau_{i+1}}^\alpha$ be the set of such points $p$. For each $p\in P_{\tau_{i+1}}^\alpha$, we invoke 
Algorithm~\ref{alg:offline-2} to report all $\tau_{i+1}$-durable triangles that contain $p$. 

 \mparagraph{Case (2.2)} We find all points $p$ with $\tau\leq \beta^{\tau_i}_p$ from $\S_\beta$.
Let $P_{\tau_{i+1}}^\beta$ be the set of such points $p$.
For each such a point $p\in P_{\tau_{i+1}}^\beta$ we invoke Algorithm~\ref{alg:report-delta-general} to report all triangles in $T_{\tau_{i+1}} \setminus T_{\tau_i}$ that contain each such a point $p$. Notice that $P_{\tau_{i+1}}=P_{\tau_{i+1}}^\alpha\cup P_{\tau_{i+1}}^\beta$. 

We run $\DTCEQ(p,\tau_{i},\tau_{i+1},\eps/2)$ and get $k=O(\eps^{-O(\ddim)})$ canonical subsets (of the cover tree in $\DTC$), $\C_p=\{\C_{p,1},\ldots, \C_{p,k}\}$.
We also partition each $\C_{p,j}$ into two different subsets of points,  $\Lambda_j^p$ and $\Psi_j^p$, as we had before and we set $\C_{p,j}=\Lambda_j^p\cup \Psi_j^p$.
We further distinguish a $\tau_{i+1}$-durable but non ${\tau_{i}}$-durable triangle $(p,q,q')$ that contains $p$ into three types: (1) $q,q' \in \Lambda^q_j$; (2) $q \in \Lambda^q_j$, $q' \in \Psi^q_j$; (3) $q \in \Lambda^q_j, q' \in \Psi^q_k$ for $j \neq k$. We only need to report triangles in type (1) when $|\Lambda_{p,j}|>1$, i.e., there are multiple points from $\C_{p,j}$ with durability threshold in $[\tau_{i+1}, {\tau_{i}})$, hence every pair in the Cartesian product of $\Lambda_{p,j} \times \Lambda_{p,j}$ must form a $\tau_{i+1}$-durable but not ${\tau_{i}}$-durable triangle with $p$. We only need to report triangles in type (2) when $|\Lambda_{p,j}|\ge 1$ and $|\Psi_{p,j}| \ge 1$, i.e., there exists a pair of points from $\C_{p,j}$ with durability threshold in $[\tau_{i+1}, {\tau_{i}})$ and $[{\tau_{i}}, +\infty)$ separately, hence every pair in the Cartesian product of $\Lambda_{p,j} \times \Psi_{p,j}$ must form a $\tau_{i+1}$-durable but not ${\tau_{i}}$-durable triangle with $p$. To report triangles in type (3) we consider any pair of canonical subsets $\C_{p,j}, \C_{p,h}$ with $h\neq j$ and $\dist(\rep_j,\rep_h)\leq 1+\eps/2$, and we report all triangles $(p,q,q')$ as long as either $q\in \Lambda_h^p\cup \Lambda_j^p$ or $q'\in \Lambda_h^p\cup \Lambda_j^p$, and $q, q'$ belong in different subsets.

At last, we update $\S_\beta$.
It suffices to compute $\beta^{\tau_{i+1}}_p$ for every point $p \in P_{\tau_{i+1}}$. We distinguish two cases for each point $p \in P_{\tau_{i+1}}$: 
\begin{itemize}[leftmargin=*]
    \item if ${\tau_{i+1}} \leq \alpha_p < {\tau_{i}}$, we compute $\beta^{\tau_{i+1}}_p$ as described at the beginning of the current subsection.
    \item otherwise, $\alpha_p > {\tau_{i}}$. We further distinguish two more cases:
    \begin{itemize}
        \item if $\beta^{\tau_{i}}_p < {\tau_{i+1}}$, we do not need to change the activation threshold for $p$, since $\beta^{\tau_{i}}_p = \beta^{\tau_{i+1}}_p$ in this case.
        \item otherwise, $\beta^{\tau_{i}}_p \geq {\tau_{i+1}}$, we compute $\beta^{\tau_{i+1}}_p$. 
    \end{itemize}
\end{itemize}

The correctness is shown in Appendix~\ref{appndx:corrMaintain}. In particular, we prove that all $\tau_{i+1}$-durable triangles and a few $\tau_{i+1}$-durable but not $\tau_{i}$-durable $\eps$-triangles will be reported. If $\OUTON$ is the output size of our algorithm in {\bf Case 2}, we have $|T_{\tau_{i+1}}\setminus T_{\tau_i}|\leq \OUTON\leq |T_{\tau_{i+1}}^\eps\setminus T_{\tau_i}^\eps|$.


\paragraph{Time Complexity.}
Both cases take $O\left(\OUTON + \eps^{-O(\ddim)}\log^2 n \right)$ time to report all ${\tau_{i+1}}$-durable triangles (but with different values of $\OUTON$), and $O(\eps^{-O(\ddim)}\log^3 n)$ time to compute $\beta^{\tau_{i+1}}_p$ for each point $p \in P_{\tau_{i+1}}$. As defined, each point $p \in P_{\tau_{i+1}}$ must participate in at least one new ${\tau_{i+1}}$-durable triangle, which is also reported in this case. Togeher, we come to:
\begin{theorem}
\label{thm:online}
  Given a metric space $(P,\phi)$ of $n$ points and $\epsilon>0$, a data structure of size $O(n\log^{2}n)$ can be constructed in $O(n\log^{3}n)$ time such that, given a parameter $\eps$, the $\epsilon$-approximate \problemtwo\ can be solved in $O\left(\OUTON \cdot \eps^{-O(\ddim)}\log^3 n\right)$ time, where $\ddim$ is the doubling dimension of $P$, and $\OUTON$ is the number of results reported. %\in \left[|T_{\tau_{i+1}}\setminus T_{\tau_i}|, |T_{\tau_{i+1}}^\eps\setminus T_{\tau_i}^\eps|\right]$. 
\end{theorem}

==> prelim.tex <==
\section{Preliminaries}
\label{sec:preliminary}

We start with some basic data structures. Then, we introduce an oracle that will be frequently used by our algorithms. We show how to combine the basic data structures to answer the oracle efficiently.

\subsection{Data structures for ball-reporting queries}
\label{subsec:structures}
Let $(P,\dist)$ be a metric space as defined earlier above. Give a point $p$, let $\mathcal{B}(p)=\{x\in\Re^d\mid \dist(x,p)\leq 1\}$ be the unit ball centered at $p$. We describe a data structure based on the \emph{cover tree}~\cite{beygelzimer2006cover, har2005fast} for answering ball-reporting queries approximately, in the sense that we report all pairs of $\mathcal{B}(p) \cap P$ but may also return some points of $\mathcal{B}(p, 1+\epsilon) \cap P$. We will use this a data structure to answer $\tau$-durable ball queries in the next subsection.

A cover tree $\mathcal{T}$ is a data structure consisting of a hierarchy of balls.
By definition, the level of the leaf nodes is the smallest one, while the level of the root node is the largest one.
Each node $u$ of $\mathcal{T}$ is associated with a representative point $\rep_u \in P$ and a ball $\mathcal{B}_u$.
If a node $u$ is at level $i$ of the tree then its children are at level $i-1$.
Let $C_i$ be the set of balls associated with nodes at level $i$.
The radius of each ball $\mathcal{B}_u$ at level $i$ is $2^i$ (notice that our definition allows levels to be positive or negative). Each point $p\in P$ is stored in one of the leaf nodes.
The root consists of a ball that covers the entire data set.
For a constant parameter $b$, a cover tree satisfies:
%
\begin{itemize}[leftmargin=*]
    \item {\bf ({Nesting})} If there is a node $u$ at level $i$ with a representative point $\rep_u\in P$, then $\rep_u$ is also a representative point in a node at level $i-1$.
    \item {\bf ({Covering})} For every representative point $\rep_u$ at level $i-1$, there exists at least one representative $\rep_v$ at level $i$ such that $\dist(\rep_v,\rep_u)<b^i$. We designate $v$ as the parent of $u$.\footnote{If there are multiple such nodes, we choose one arbitrarily.}
    \item {\bf ({Separation})} For any $\rep_u, \rep_v$ at level $i$, $\dist(\rep_u,\rep_v)>b^i$.
\end{itemize}

W.l.o.g. assume $b=2$.
In the literature, a cover tree %(or net tree) 
was mostly used for approximate nearest-neighbor queries. In Appendix~\ref{appndx:covertree}, we show how to construct a modified cover tree with space $O(n\log n)$ in $O(n\log n)$ time, while achieving the following guarantees when the spread is bounded. For a query point $q\in\Re^d$, it returns a set of $O(\log n + \eps^{-O(\ddim)})$ canonical balls of diameter $\eps$, possibly intersecting, such that each point of $\mathcal{B}(q)\cap P$ belongs to a unique canonical ball. Each canonical ball may contain some points of $\mathcal{B}(q, 1+\epsilon) \cap P$.


%For ball queries under the $\ell_\infty$ metric, instead of a cover tree, we use a \emph{range tree}~\cite{mark2008computational} to return $\mathcal{B}(q) \cap P$ exactly as the union of $O(\log^d n)$ canonical subsets since an $\ell_\infty$-ball is a hypercube. For ball-reporting queries in any $\ell_\alpha$ norm, we can use a \emph{quad-tree}~\cite{agarwal2017range}.
%The preprocessing time, space usage and query time of these classical data structures are summarized in Table~\ref{tab:data_structure}. %We use the range trees and the quadtrees with a similar way they are used in the literature for range reporting queries~\cite{agarwal2017range}.
%On the other hand, cover-trees have mostly been used for approximating the nearest neighbor query~\cite{beygelzimer2006cover, har2005fast}.
%In Appendix~\ref{appndx:dataStructures}, we show the complexities of these data structures. %and also show how we can use a cover tree to approximately answer reporting queries when the spread is bounded. 

%In particular, we construct a modified cover tree of size $O(n\log n)$ in $O(n\log n)$ time such that, given a query point $q$ and a parameter $\eps$ we can find $O(\eps^{-O(\ddim)})$ canonical subsets that contain all points within distance $1$ from $q$ and might contain points with distance $1+\eps$ from $q$. Furthermore, we can argue that each pair of points in a canonical subset has distance at most $\eps$.


\subsection{$\tau$-durable ball query}
\label{sec:tau-durable-ball}
%Ideally, we would like to solve the following query.
\begin{definition}[$\tau$-durable ball query]
    Given a metric space $(P,\dist)$, $\tau > 0$ and a point $q$ with time interval $I_q$, it asks to return all points $p \in P$ such that $\dist(p,q) \le 1$, $|I_p \cap I_q| \ge \tau$, and $I_q^- \in I_p$. 
\end{definition}

Answering such a query exactly is inherently expensive even in the Euclidean space, since a near-linear space data structure has $O(n^{1-1/d}\log n + \OUT)$ query time~\cite{chan2012optimal}, where $\OUT$ is the output size. Instead, we consider the following relaxed version: %with an approximation on the distance requirement: 

\begin{definition}[$\eps$-approximate $\tau$-durable ball query]
    Given a metric space $(P,\dist)$, $\tau > 0$, $\eps > 0$, and a point $q$ with time interval $I_q$, it asks to report a subset $Q \subseteq P$ of points such that $\mathcal{B}(q) \cap P \subseteq Q \subseteq \mathcal{B}(q, 1+\epsilon) \cap P$, and for any $p \in Q$, $|I_p \cap I_q| \ge \tau$ and $I_q^- \in I_p$. 
\end{definition}

Intuitively, we use a multi-level data structure to handle this query.
In the first level, we use a cover tree to find a small number of canonical subset that contain the points of $\mathcal{B}(q) \cap P$ (but may also contain some point of $\mathcal{B}(q, 1+\epsilon) \cap P$). At each node of the cover tree, we also construct an \emph{interval tree}~\cite{mark2008computational} over the intervals of the points stored at this node. An interval tree is a data structure that can answer intersection queries of a query interval with the set of intervals stored in the interval tree. Using the cover tree along with interval trees, we can find a set of canonical nodes that contain all points within distance $1$ from $q$ and $I_q^-\in I_p$, but they may also contain points within distance $1+\eps$ from $q$.

More specifically, we construct a cover tree $\CT$ over $P$. For each node $u$ of $\CT$, we further construct an interval tree $\IT_u$ over the intervals of points lying in the ball defined by $u$. Recall that each node $u_i$ of $\CT$ is associated with a representative point $\textsf{rep}_i\in P$.
Let $\DTC$ be the data structure built for $P$. The data structure $\DTC$ uses $O(n\log n)$ space and can be constructed in $O(n\log^2{n})$ time. Let $\DTCQ(p, \tau, \eps)$ denote the query procedure of $\DTC$ with  parameters $p, \tau, \eps$. This query can be answered as follows:
\begin{itemize}[leftmargin=*]
    \item {\bf (step 1)} We first query the $\CT$ with point $p$ and radius $r = 1$, and will obtain a canonical subset of nodes $\mathcal{C}=\{u_1, u_2, \ldots, u_k\}$ for $k = O(\eps^{-\ddim})$. From Appendix~\ref{appndx:covertree}, we have that each node in $\mathcal{C}$ corresponds to a ball of radius $\eps/2$. Furthermore, for each $u_j\in \mathcal{C}$,  $\dist(p,\textsf{rep}_j)\le 1+\eps/2$.
    \item {\bf (step 2)} For each canonical node $u_j \in \C$, we query the $\IT_{u_j}$ with $I^-_p$, and will obtain all $q \in \IT_u$ such that $I_q^- +\tau\leq I_p^- +\tau\leq I_q^+$. 
\end{itemize}
Note that $\DTC$ might return a point $q$ such that $\dist(p,q) > 1$, but $\dist(p,q) < 1+\eps$ always holds. Together, we obtain:

\begin{lemma}
\label{lem:helper-2}
    A data structure can be built in $O(n\log^2 n)$ time with $O(n\log n)$ space, such that any $\eps$-approximate $\tau$-durable ball query can be answered in $O(\eps^{-O(\ddim)}\log n)$ time.
\end{lemma}

%All our algorithms consider each point $q\in P$ one by one and uses such a data structure to report all $\tau$-durable patterns such that $q$ is the newest point with respect to the associated time intervals ($I_q^-\in I_p$ for each $p$). In this way we make sure that each durable pattern is reported once.
\paragraph{Remark.} The data structure $\DTC$ can also be extended to support finding durable triangles with other linear constraints on the endpoints of the intervals, say $I_p^- \le I_q^- \le I_p^+\leq I_q^-+\tau'$ for some $\tau' >0$. Let $\DTCE$ be the extended version of $\DTC$, containing a cover tree and then interval trees in the next levels.
Let also $\DTCQ(p,\tau,\tau',\eps)$ denote the query procedure of the extended data structure, where $\tau, \tau'$ are two durability parameters that are used to search $\DTCE$.
The space, construction time and query time of $\DTCE$ are increased only by a $\log n$-factor compared with $\DTC$.
